Audio-Visual Speaker Diarization Based on Spatiotemporal Bayesian Fusion

Speaker diarization consists of assigning speech signals to people engaged in a dialogue. An audio-visual spatiotemporal diarization model is proposed. The model is well suited for challenging scenarios that consist of several participants engaged in multi-party interaction while they move around and turn their heads towards the other participants rather than facing the cameras and the microphones. Multiple-person visual tracking is combined with multiple speech-source localization in order to tackle the speech-to-person association problem. The latter is solved within a novel audio-visual fusion method on the following grounds: binaural spectral features are first extracted from a microphone pair, then a supervised audio-visual alignment technique maps these features onto an image, and finally a semi-supervised clustering method assigns binaural spectral features to visible persons. The main advantage of this method over previous work is that it processes in a principled way speech signals uttered simultaneously by multiple persons. The diarization itself is cast into a latent-variable temporal graphical model that infers speaker identities and speech turns, based on the output of an audio-visual association process, executed at each time slice, and on the dynamics of the diarization variable itself. The proposed formulation yields an efficient exact inference procedure. A novel dataset, that contains audio-visual training data as well as a number of scenarios involving several participants engaged in formal and informal dialogue, is introduced. The proposed method is thoroughly tested and benchmarked with respect to several state-of-the art diarization algorithms.

==> coverletter_Aug-2016.tex <==
\pagestyle{empty}
\onecolumn

\begin{coverletter}{Audio-Visual Speaker Diarization Based on Spatiotemporal Bayesian Fusion}{TPAMISI-2016-03-0203}

\begin{answereditor}{There are no comments from the editor.} 
We would like to thank the two reviewers for their interesting comments, remarks, and suggestions. We carefully revised the paper accordingly. Below we answer in detail the comments and questions of the reviewers. 
The changes made to the paper can be easily tracked by following the cross references incorporated in our answers, for example  \refcm{multiple-speech} refers to paragraph C4 on page~3. Below we summarize the list of revisions:
\begin{itemize}
\item We clarify several issues that seemed to be miss-understood by Reviewer 1, in particular: the originality of our method with respect to existing diarization methods and the originality of our visually-guided multiple speech-source localization with respect to several sound-source localization algorithms and with respect to [33].
\item We clarify the use of the visual tracker which is not assumed to provide a perfect output, as wrongly interpreted by Reviewer 1 (see our response below and \refcm{visual-tracking}). 
\item In response to Reviewer 1, we clarify that our method requires that a person is considered only if he/she is both seen and heard. A person lying outside the camera field of view is not taken into account, \refcm{state-transition-1} and \refcm{state-transition-2}.
\item We completely revised Section \ref{sec:experiments}: our diarization method is now compared with four other methods, \refcm{comparisons-1}, while our sound-source localization method is compared with two state-of-the-art methods, \refcm{comparisons-2}. We provide a detailed discussion concerning the results obtained with four datasets \refcm{discussion-1}, \refcm{discussion-2}, \refcm{discussion-3}, \refcm{discussion-4}, and \refcm{discussion-5}. 
\end{itemize}
\end{answereditor}

\begin{answerreviewer}[Recommendation: Author Should Prepare A Major Revision For A Second Review]
\ca{I am a bit unsure whether the technical contribution in this manuscript is at TPAMI standards. The speaker diarization model is based on common design choices in the bayesian filtering framework. The audio observation model is based on binaural features that have interesting properties well studied in the recent paper [33]%\cite{deleforge2015colocalization}.
} 
{
The paper addresses the problem of speaker diarization using both audio and visual observations. The proposed method overcomes two major limitations of existing diarization techniques: (i) it considers complex scenarios where participants do not always face the cameras, move around, leave or enter the room, presence of non-speech sounds, etc. (ii) it allows overlapping speech signals. We propose a novel diarization formulation based on jointly observing visual and auditory features and on associating them at each frame, rather then using long sequences of past, present and future frames. The Bayesian filtering framework offers several possible modeling schemes. We are aware of only one such scheme that specifically addresses multimodal diarization, namely [3]. We discuss in detail our original contribution with respect to [3]. In particular the model of [3] is non-causal (it requires future information to take decisions), it can deal neither with complex and dynamic scenes, nor with overlapping speech. In this paper we do not use the method of [33] which is not specifically designed to locate speech sources and which does not take into account the sparsity of speech signals in the Fourier domain. Nevertheless, we do borrow from [33] the idea of learning a mapping between binaural features and the location of a sound source in the image.
}

\ca{It is also unclear whether the approximation in \eref{eq:cross-psd} - \eref{eq:cross-psd-one} leading to the actual definition of binaural feature vector in \eref{eq:RTF-one} is novel or a non-trivial choice. The spectral sparsity argument is common and practical in case of speech but leads to a rather straightforward extension to a multi-speaker situation (pg 3 l.30-52).} 
{Equations (10)-(12) hold only for the case of a single speech signal corrupted by noise. One can notice that the binaural features defined by (12) are obtained by averaging over several audio frames (indexed by $k$). These equations cannot be directly used for the case of multiple speakers but they do help to understand the difficulty associated with their generalization to simultaneously-emitting speech sources. Indeed, in the latter case, one cannot average the binaural features over several frames because the non-stationary nature of speech in general (Notice the important difference between the time index $t$ and the audio-frame index $f$. An audio-visual time window $t$ is composed of several audio frames, as explained in Section III, second paragraph). One may also remark that multiple speaker localization is far from being a solved problem in the audio signal processing literature. \textbf{We added three recent references [25, 26, 27] as well as a paragraph in the state of the art section, \refcm{multiple-speech}}. A complete review of these methods is out of the scope of this paper. In general, multiple speaker localization methods are \textit{semi-blind}, namely the number of sources to be located is known in advance. Here we propose to solve this problem by combining audio and visual information, as explained in detail in Section VI. To conclude, Section V describes the binaural features that we use, while the problem of multiple speech-source localization itself is addressed in Section VI. 
}

\ca{The audio-visual fusion assumes the visual tracking is exact by an external method while this may not be the case in challenging scenarios. In a realistic multi-person scenario visual tracking is challenging and there is no evidence that the proposed method be robust to tracking inaccuracies. And it is not unlikely that a person be hidden by another in the camera while speaking, and this is a condition that is violated in the state transition model \eref{eq:transition-cases}.}
{
It is not assumed that the (external) visual tracker is exact. Some state-of-the-art multi-person visual trackers estimate a trajectory for each person under the form of a state variable with its dynamics. A binary control variable is associated with each tracked person. When a person is not detected in a frame for various reasons (out of field of view, occlusions, bad lighting, detection failure, etc.), this variable is set to 0. Please refer to Section III, first paragraph as well as to Figure 1. We added a paragraph at the end of Section~\ref{sec:visual} that provides additional details about the visual tracker, \refcm{visual-tracking}.

We revised Section~\ref{sec:state-transition}. We added a paragraph that briefly mentions turn-taking methods existing in the literature, \refcm{turn-taking}. We also added a paragraph that recalls that our \textbf{audio-visual} diarization model requires that a person is both seen and heard to be qualified as an ``active speaker", and an explanation about the proposed transition model, \refcm{state-transition-1} and \refcm{state-transition-2}.
} 

\ca{It is however a nice property that the method can make use of white-noise single source training samples and generalize well to multi-speaker scenario as demonstrated by the experiments. It requires however a dense set of training samples, \fref{fig:dataset_setup_b}, which is costly to acquire.}
{It takes approximately ten minutes to acquire a set of training samples for each source-to-camera distance.}
\qa{All parameter values should be given for the experiments - e.g. what is the value of threshold ``a" in (16) ? What is the value of the self-transition prior ``q" in (7) ? How is that values obtained ?}
{The adaptive threshold $a$ is estimated based on noise statistics \refcm{adaptive-th}. The value of $q$ is estimated experimentally \refcm{state-transition-1}.}
\qa{Is \eref{eq:RTF-one} symmetric, i.e., is $\phi_{L,R} / \phi_{RR} = \phi_{R,L} / \phi_{LL} $. Why not using $\phi_{L,R} / \phi_{RR} + \phi_{R,L} / \phi_{LL}$ in \eref{eq:RTF-one} and \eref{eq:RTF-several} ?}
{Indeed, in \eref{eq:RTF-one} one can use either $\phi_{L,R} / \phi_{RR}$ or $\phi_{R,L} / \phi_{LL} $ but the two expressions yield either a positive or a negative phase difference between the two microphone signals, respectively. A phase difference in the spectral domain corresponds to a time difference of arrival (TDOA) between the left and right microphones, and hence to a sound direction. The choice of either one of these ratios is well documented in [40]. Nevertheless, one needs to make a consistent choice (left/right or right/left) over all the frames and over all the frequencies. 
}
\qa{In the tables II to V it would be nice to add a row with an overall score on each dataset, e.g. DER averaged over all dataset sequences for each method}
{We added a row with the average DER on each dataset.}
\qa{Few typos: "the the" at p6 L53 , "benchamrk" at p6 L37 , "Table III" at p10 L18 should probably be "Table II" ; "1circ" should probably be "1\~circ" at p10 L37 ; "Citeseer" in citation 
%\cite{garau2010audio}.
}
{Done}
\end{answerreviewer}

\begin{answerreviewer}[Recommendation: Author Should Prepare A Major Revision For A Second Review]
\ca{This paper proposes a speaker diarization problem based on both audio and visual signal. There are some questions and concerns needs to be addressed.}
{We tried to address all the concerns raised by the reviewer.}
\qa{Compared with audio observation model, the visual part is a little poor. In section IV, the authors only use one paragraph to describe their visual observation approach. Based on my understanding, the visual information is also important for the proposed problem. Please enhance the visual part in the revision, such as using head pose cues, person positioning cues, etc.}
{As already explained above (please consult our responses to Reviewer 1) the multi-person visual tracker is somehow external to the method proposed in this paper. As mentioned by Reviewer 1, visual tracking has lots of inaccuracies and this indeed is formally taken into account by our formulation. It is an excellent idea to incorporate head-pose cues, person positioning cues, and the like. Unfortunately these methods come with their inaccuracies as well and overall, they may have the undesirable effect of downgrading the performance of our diarization method. Notice that in this paper we address the problem of assigning speech segments to participants and not the problem of estimating who speaks to whom, which indeed would require analysis of person-to-person interactions. We added a sentence in the conclusions and we cite these two papers \refcm{camera-network}.}
\qa{The experiments are weak. The provided baselines are not enough. The authors should compare with different fusion strategies, multi-modal/multi-view/multi-task approaches, etc.}
{Audio-visual fusion is a special case of sensor fusion and there is no general-purpose sensor-fusion methodology that can be applied to audio-visual fusion. More specifically, audio signals are usually described and analyzed in spectral domains, e.g. STFT, MFCC, etc., while visual information is usually described in the image domain or in some feature spaces. The fusion strategy adopted in this paper is based on probabilistic association between 2D visual features (positions of faces) and high-dimensional spectral features. We believe that the proposed fusion strategy (Section VI) is an original contribution on its own. The vast majority of the baseline methods [2], [3], [9], [10], [11], [12], [13], and [21] perform fusion based on temporal correlation between audio features and visual features. We implemented one of these methods ([21)] and compared it with our method as well as with other methods. One should however keep in mind that these methods (based on audio-visual temporal correlation) assume very simple scenarios (static people facing the cameras), and require long sequences, hence they cannot be applied to all the dataset recordings used in this paper. 

To take into account this comment, we completely revised Section \ref{sec:experiments}: the proposed method is now compared with four other methods \refcm{comparisons-1}. We also added two other sound-source localization methods  and we combine these methods with our diarization algorithm \refcm{comparisons-2}.
}
\qa{Please analyze the complexity of the proposed approach.}
{The complexity of the proposed Bayesian model is discussed in \refcm{complexity}.}
\qa{The authors should discuss the following related paper for the informal scenarios analysis: \\
a. Analyzing Free-standing Conversational Groups: a Multimodal Approach, ACM Multimedia 2015 \\
b. No matter where you are: Flexible graph-guided multi-task learning for multi-view head pose classification under target motion, TPAMI 2016}
{The multimodal method of the first one of these papers makes use of both wearable and distributed sensors. Our paper address a different sensor architecture, namely both the cameras and the microphones are placed on an artificial \textit{agent} such as a robot. The second one of these papers addresses the problem of head-pose classification using a distributed camera network. Both these papers address complex scenarios with many (tens) of people, while our method is merely limited to scenarios with a few (less than ten) people, as encountered in human-robot and human-computer interaction. We added a short sentence at the end of the paper to emphasize possible extensions of our approach \refcm{camera-network}. }
\qa{Overall, the paper proposes an interesting and useful problem. However, the experiments are not enough for a TPAMI paper. Please provide more experiments to prove the effectiveness of their approach in the revision.}
{We took this comment very seriously and we completely revised the experimental section. Please consult the following new/revised paragraphs: \refcm{comparisons-1}, \refcm{comparisons-2}, \refcm{discussion-1},  \refcm{discussion-2}, \refcm{discussion-3}, \refcm{discussion-4}, \refcm{discussion-5}.}
\end{answerreviewer}


\end{coverletter}

\twocolumn
\setcounter{page}{1}
